Self-Alignment Pretraining for Biomedical Entity Representations

Despite the widespread success of self-supervised learning via masked language models (MLM), accurately capturing fine-grained semantic relationships in the biomedical domain remains a challenge. This is of paramount importance for entity-level tasks such as entity linking where the ability to model entity relations (especially synonymy) is pivotal. To address this challenge, we propose SapBERT, a pretraining scheme that self-aligns the representation space of biomedical entities. We design a scalable metric learning framework that can leverage UMLS, a massive collection of biomedical ontologies with 4M+ concepts. In contrast with previous pipeline-based hybrid systems, SapBERT offers an elegant one-model-for-all solution to the problem of medical entity linking (MEL), achieving a new state-of-the-art (SOTA) on six MEL benchmarking datasets. In the scientific domain, we achieve SOTA even without task-specific supervision. With substantial improvement over various domain-specific pretrained MLMs such as BioBERT, SciBERTand and PubMedBERT, our pretraining scheme proves to be both effective and robust.

==> backups/abstract.tex <==
\begin{abstract}

% Medical concept normalisation (MCN), i.e. the task of mapping medical mentions to a well-defined knowledge graph, is currently tackled with hybrid systems using both string-matching based heuristics and Transformer-based neural language models using many different pre-training techniques and loss functions.
% In this paper we try to shed light on this process by investigating best practices for fine-tuning purely neural MCN models; we evaluate pre-training on the UMLS methatesaurus and the use several loss functions.
% We show that framing MCN as a metric lerning problem allows us to obtain results on par with current hybrid string-matching/neural SOTA models without any specific fine-turning. After fine-tuning on specific datasets, our model can easily outperform SOTA models by large margins.

% \fl{I like this new framing. I think one more thing that needs to be pointed out is the metric learning pre-training stage is essential for our model (Other papers take off-the shelf xxBERT as the neural model). And this pre-training alone is on par with SOTA.}

%% OLD %%
Medical concept normalisation (MCN) is a task of mapping \zm{the medical mentions into the unified concepts in a medical} knowledge graph. State-of-the-art (SOTA) systems tackle \zm{this task} with hybrid components leveraging both string-matching based heuristics and Transformer-based neural language models. In this work, we propose a simple yet powerful pre-trained Transformer-based model, \zm{called} SapBERT (\textbf{S}elf-\textbf{a}ligning \textbf{p}retrained \textbf{BERT}), that easily outperforms prior systems on a variety of MCN benchmarks without finetuning on any data sets\zmc{Do we finetune in the three social media datasets?}. Compared with other pretrained models such as BioBERT, SciBERT, our proposed SapBERT provides the best pretraining scheme for MCN, outperforming the competitors by up to +20\% top-1 accuracy. The success of our model is attributed to: (1) language model pre-training on UMLS to discover knowledge stored in very large-scale structured data; (2) unifying the language model pre-training and MCN with the same metric learning objective that clusters synonyms through self-alignment. We provide thorough ablation studies and qualitative analysis to shed light on where the improvement comes from.
%\fl{I wrote another version of abstract. This should be a more accurate illustration of the experiments I've done.}



%%%%%% Zaiqiao %%%%%%
% Title: SnapBERT: Self-aligning pre-trained BERT for Medical Concept Normalisation
% I still keep the original ones.
%\zm{With the capability of modelling bidirectional contexts, masked language models pre-trained with a domain-specific corpora (such as SciBERT and BioBERT) achieve better performance in the biomedical mining tasks than these models pre-traprined with a general domain corpora (e.g. the vanilla BERT). However, in the Medical Concept Normalisation (MCN) task, the word-masked pre-training scheme adopted by these models that predicts randomly masked words in a sequence still neglect the rich synonyms among the biomedical concepts. In this work, we propose a powerful augmented pre-training scheme for BERTs, namely the \textbf{S}elf-\textbf{a}ligning \textbf{p}retrained \textbf{BERT} (\textbf{SapBERT}), that further pre-trains a existing BERT to self-align concepts using the UMLS corpora with  a metric learning loss. Our experimental results conduct in five MCN datasets show that, this simple augmented pre-training scheme can significantly outperform several popular biomedical-specified pre-trained BERTs, such as BioBERT, SciBERT and PubMedBERT, in terms of the effectiveness by up-to 30\%? improvement under top-1 accuracy.}

\end{abstract}

==> backups/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

==> backups/discussion.tex <==
\section{Discussion}\label{sec:discussion}
\stitle{generalise to other/general domains.}

\stitle{generalise to other BioNLP tasks} e.g. MedNLI.

\stitle{phrase to sentence level.} current model on phrase level $->$ needs to extend to sentence level.

\stitle{take hierarchical information into account} \citep{murty2018hierarchical}

==> backups/experiment.tex <==
\section{Experiment}\label{sec:experiment}

Please refer to appendix for data pre-processing of UMLS synonyms and training details.

\subsection{Training details}
For hyper-parameters of online mining, we use $\lambda=0.2$ which is the same as \citet{schroff2015facenet}; for MS loss, we use the default ones from \citet{wang2019multi}. For the margin of triplet loss, we use the default value from PyTorch. For pre-training, all models are trained with AdamW with learning rate of 2e-5 for 1 epoch with a batch size of 480. To ensure that enough positive samples are presented in each mini-batch, instead of completely random batching, we prepare generate a positive pair list offline - so that 240 positive pairs are batched for each iteration. Specifically, for each concept, we enumerate the combinations of its synonyms as positive pairs. To ensure balanced number of samples from each concept, we randomly choose 50 pairs if the generated positive pairs are more than 50. In total, around 50k iterations are performed during the pre-training. For finetuning, we do the same as pre-training but now the positive pair list is generated from the concatenation of training data and reference ontology. And we train for 15 epochs with a batch size of 256.

\subsection{Datasets}


\subsection{Main results}
compare umls-bert \& umls-bert (finetued) with all sota results.


% \begin{table*}[]
%     \centering
%     \scriptsize
%     \hspace*{-1cm}
% \begin{tabular}{llcccccccccccccccccccc}
% \toprule
% \multirow{2}{*}{\#} & \multirow{2}{*}{model} & \multicolumn{2}{c}{cometa sf.g.} & & \multicolumn{2}{c}{cometa zs.g.} & &\multicolumn{2}{c}{ncbi dis.} &  &\multicolumn{2}{c}{bc5cdr dis.} &  &\multicolumn{2}{c}{bc5cdr che.}  & 
% & \multicolumn{2}{c}{TwADR} & 
% & \multicolumn{2}{c}{AskAPatient} \\
% \cmidrule[1.5pt]{3-4}\cmidrule[1.5pt]{6-7}\cmidrule[1.5pt]{9-10}\cmidrule[1.5pt]{12-13}\cmidrule[1.5pt]{15-16}\cmidrule[1.5pt]{18-19}\cmidrule[1.5pt]{21-22}
% & & a@1 & a@5 & & a@1 & a@5 & & a@1 & a@5 & & a@1 & a@5 & & a@1 & a@5 & & a@1 & a@5 & & a@1 & a@5 \\
% \hline
% 3.1 & BioSyn \citep{sung2020biomedical} & .713 & .778 & &.65 & .76 & & .911 & .939 & & \textbf{.932}  & \textbf{.960} & & \textbf{.966} & .972\\
% 3.2 & Gen-Rank \citep{xu-etal-2020-generate} & - & - & & - & - & & & & & & & & & & & .470 & - & & .875 & - \\
% \hline
% 3.3 & BioBert & & & & & & & & & & & & & & & &  & - & & .414 & .514 \\
% 3.4 & - finetuned & & & & & & & & & & & & & & & &  & - & & .877 & - \\
% \hline 
% 3.5 & UMLS Bert v1.0 & .637 & .753 & & \textbf{.66} & \textbf{.78} & &  .910 & .947 & & .931 & .956 & & .965 & \textbf{.977} & &   & - & & .724 & -  \\
% 3.6 & - finetuned & \textbf{.756} & \textbf{.844} & & .654 & .770 & &  \textbf{.923} & \textbf{.954} & & & & &  &  & &  & - & & \textbf{.892} &\\
% \bottomrule
% \end{tabular}
%     \caption{UMLS Bert (unsupervised) vs. SOTA.}
%     \label{tab:my_label}
% \end{table*}


\begin{table*}[]
\setlength{\tabcolsep}{1.5pt}
    \centering
    \small
%\hspace*{-1.5cm}
\begin{tabular}{llccccccccccccccccc}
\toprule
\multirow{2}{*}{\#} & \multirow{2}{*}{model} & \multicolumn{2}{c}{ncbi dis.} &  &\multicolumn{2}{c}{bc5cdr dis.} &  &\multicolumn{2}{c}{bc5cdr che.} & & \multicolumn{2}{c}{MedMentions} \\
\cmidrule[1.5pt]{3-4}\cmidrule[1.5pt]{6-7}\cmidrule[1.5pt]{9-10}\cmidrule[1.5pt]{12-13}
& & top-1 & top-5 & & top-1 & top-5 & & top-1 & top-5 & & top-1 & top-5  \\
\hline
& Sieve-Based \scriptsize \citep{d2015sieve} &  84.7 & - & & 84.1 & - & & 90.7 & - & & -&-\\
& TagegrOne \scriptsize \citep{leaman2016taggerone} &  87.7 & - & & 88.9 & - & & 94.1 & - &  & -&- \\
& NormCo \scriptsize \citep{wright2019normco} & 87.8 & - & & 88.0 & - &  & -&-&  & -&-\\
& BNE \scriptsize  \citep{phan2019robust} & 87.7 & -  & & 90.6 & - & & 95.8 & - &  & -&- \\
& BertRank\scriptsize \citep{ji2020bert} & 89.1 & - &  & -&-&  & -&-&  & -&-\\
 & BioSyn \scriptsize \citep{sung2020biomedical} & 91.1 & 93.9 & & 93.2  & \textbf{96.0} & & \textbf{96.6} & 97.2 & & \multicolumn{2}{c}{Out-Of-Mem.}\\
\hline
 & \multirow{2}{*}{SapBert \scriptsize (PubMedBert as base)} & \underline{\textbf{92.0}} & \underline{\textbf{95.6}} & & \underline{\textbf{93.5}} & \textbf{96.0} & & 96.5 & \underline{\textbf{98.2}} &  & 51.1 & 74.5 \\
 & & \scriptsize ($\pm$0.2) & \scriptsize ($\pm$0.2) & & \scriptsize ($\pm$0.2) &\scriptsize ($\pm$0.2) & & \scriptsize ($\pm$0.2) & \scriptsize ($\pm$0.2) \\
\bottomrule
\end{tabular}
    \caption{\small SapBert (unsupervised) vs. SOTA (supervised). The reported SapBert model results are average of five runs of pre-training with five different random seeds. ``$(\pm\ \cdot)$'' denotes standard deviation. Underline indicates a statistically significant better performance than the previous highest scores
(T-test with p-value $<0.05$). ``$\ast$'' denotes results produced using official released code. ``-'' denotes results not being reported in the cited paper. Note that most entries in the COMETA and MedMentions are empty. COMETA is a recently relesed data set. We replicated BioSyn and tested it on COMETA. MedMentions is not attempted before likely to be a result of its massive scale. According to our experiments, BioSyn encounters OOM on our work station with 200GB RAM. According to \citet{mohan2018medmentions}, when they trained TaggerOne \citep{leaman2016taggerone} one a subset of MedMentions, it took 9 days and 900GB RAM.
}
    \label{tab:sap_bert_vs_sota}
\end{table*}

\begin{table}[]
\setlength{\tabcolsep}{2.0pt}
    \centering
    \small
\hspace*{-1.5cm}
\begin{tabular}{llllllllllllllllll}
\toprule
\multirow{2}{*}{\#} & \multirow{2}{*}{model} 
& \multicolumn{2}{c}{AskAPatient} & 
& \multicolumn{2}{c}{cometa sf g} \\
\cmidrule[1.5pt]{3-4}\cmidrule[1.5pt]{6-7}
& & top-1 & top-5 & & top-1 & top-5  \\
\hline
& WordCNN \scriptsize \citep{limsopatham-collier-2016-normalising} & 81.4 & - & & - & - \\
& WordGRU+TF-IDF \scriptsize  \citep{tutubalina2018medical} &  85.7 & - & & - & -   \\
  & BioSyn \citep{sung2020biomedical} & & & & 71.3 & 77.8 \\
  & Gen-Rank \citep{xu-etal-2020-generate} & 87.5 & -  & & -  & - \\
\hline 
 %& SapBert \scriptsize (PubMedBert as base) & 72.2  & 88.2 & &   &  \\
   &  \multirow{2}{*}{\shortstack[l]{SapBert \\ \scriptsize (PubMedBert as base; unsupervised)}} & 72.2 & 88.2 & &  63.7 & 75.3 \\
\\
  &  \multirow{2}{*}{\shortstack[l]{SapBert \\ \scriptsize (PubMedBert as base; finetuned)}} & \textbf{89.0} & \textbf{96.2} & &  \textbf{75.6} & \textbf{84.4} \\
  & & \scriptsize $(\pm)$ & \\
\bottomrule
\end{tabular}
    \caption{SapBert vs. SOTA on social media language MCN datasets. }
    \label{tab:sap_bert_finetuned}
\end{table}



Our pre-trained model is on par with sota on most of the datasets. After finetuning on scientific language datasets (ncbi, bc5cdr), the results remain similar or improve very little. After finetuning onsocial media language datasets (cometa, TwADR, AskAPatient), the performance is boosted a lot.

\subsection{Compare various base models}
Note that when computing scores of the original BERT/BioBert/PubMedBert... we directly used the \texttt{[CLS]} token representation as well. The original BERT paper argues that \texttt{[CLS]} is not meant to be used without finetuning and average of all tokens' representation might be the de-facto choice for using BERT to produce sentence representation. However, we observed lower top-1 accuracy with the averaging approach. We suspect that it is due to the length of biomedical names are not as long as sentences - so that \texttt{[CLS]} is fairly clean and accurate representation of the input while on the sentence-level, \texttt{[CLS]} struggles to capture information from long context. \fl{just an engineering note. Maybe move to appendix.}


\subsection{Compare metric learning objectives}
\textbf{TODO:}\\
1. do ablation studies on different parts of the metric learning framework: drop data mining phase \\



\begin{table}[]
    \centering
\begin{tabular}{llccccccccccccc}
\toprule
\# &  &  top-1 & top-5 \\
\hline
& w/o miner & 91.8 & 94.1 \\
& w/ miner & 93.5 & 95.7 \\
\bottomrule
\end{tabular}
    \caption{Compare w/ and w/o online mining. Test on NCBI-disease.}
    \label{tab:my_label}
\end{table}


2. try other losses, e.g. triplet loss; try different sampling strategies



\begin{table*}[]
\setlength{\tabcolsep}{2.0pt}
\centering
\begin{tabular}{llccccccccccccc}
\toprule
\# & objective &  top-1 & top-5 \\
\hline
& Cosine loss & .863 & .908 \\
& Triplet loss & .849 & .923 \\
& Contrastive loss & .852 & .927 \\
& NCA loss \citep{goldberger2005neighbourhood} & .721 & .794 \\
& InfoNCE loss (batch size 128) \citep{oord2018representation} &  .851 & .929 &  \\
& LiftedStructure loss (batch size 128) \citep{oh2016deep} &  .815 & .926 &  \\
& FastAP loss \citep{cakir2019deep} & .902 & .931 \\
& Circle loss \citep{sun2020circle} & \textbf{.904} & .939 \\
& MS loss \citep{wang2019multi} & \textbf{.904} & \textbf{.944} \\
\bottomrule
\end{tabular}
    \caption{Comparing learning objectives on a subset (100k) of UMLS synonyms. All number are produced on NCBI-disease testing set. The details of the baselines can be found in appendix.}
    \label{tab:my_label}
\end{table*}

\subsection{Domain is important (as reflected in the results)}

Without self-aligning pre-training, ClinicalBert performs the best on AskAPAtient, which is a social media language data set. After self-alignment pre-training, SapBert (BlueBert-base) performs the best on COMETA, which is a social media language data set. These results make sense as ClinicalBert and BlueBert are the only ones trained on Clinical notes, which contain large amounts of non-standard expressions like abbreviations.


\begin{table*}[]
\setlength{\tabcolsep}{2.0pt}
    \centering
    \small
%\hspace*{-1.5cm}
\begin{tabular}{llccccccccccccccccccc}
\toprule
%\# & model &  top-1 & top-5 \\
\multirow{2}{*}{\#} & \multirow{2}{*}{model} & \multicolumn{2}{c}{ncbi dis.} &  &\multicolumn{2}{c}{bc5cdr dis.} &  &\multicolumn{2}{c}{bc5cdr che.} &  &\multicolumn{2}{c}{AskAPatient} & 
& \multicolumn{2}{c}{cometa sf g} & & \multicolumn{2}{c}{MedMentions} \\
\cmidrule[1.5pt]{3-4}\cmidrule[1.5pt]{6-7}\cmidrule[1.5pt]{9-10}\cmidrule[1.5pt]{12-13}\cmidrule[1.5pt]{15-16}\cmidrule[1.5pt]{18-19}
& & top-1 & top-5 & & top-1 & top-5 & & top-1 & top-5 & & top-1 & top-5  & & top-1 & top-5 & & top-1 & top-5  \\
\hline
& BERT \citep{devlin2019bert} & 67.6 & 77.0 & &  81.4 & 89.1 & & 79.8 & 91.2 & & 38.2 & 43.3 &  & 40.4 & 47.7 & & 39.6 & 60. 2 \\
& BioBERT v1.1 \citep{lee2020biobert} & 71.3 & 84.1 & & 79.8 & 92.3 & & 74.0 & 90.0 & & 41.4 & 51.5 & & 35.9 & 46.1 & & 24.2 & 38.5\\
& BioClinicalBERT \citep{alsentzer-etal-2019-publicly} & 72.1 & 84.5 & & 82.7 & 91.6 & & 75.9 & 88.5 & & \textbf{43.9} & \textbf{54.3} & & 43.1 & 51.8 & & 40.6 & 61.8  \\
& BlueBERT \citep{peng2019transfer} & 75.7 & 87.2 & & 83.2 & 91.0 & & 87.7 & 94.1 & & 41.5 & 48.5 & & 42.9 & 52.9 & & 41.6 & 61.9 \\
& SciBERT \citep{Beltagy2019SciBERT} & \textbf{85.1} & \textbf{88.4} & & \textbf{89.3} & 92.8 & & \textbf{94.2} & \textbf{95.5} & & 42.3 & 51.9 & & \textbf{48.0} & \textbf{54.8} & & \textbf{45.8} & \textbf{66.8} \\
& PubMedBERT \citep{pubmedbert} & 77.8 & 86.9 & & 89.0 & \textbf{93.8} & & 93.0 & 94.6 & & 42.5 & 49.6 & & 46.8 & 53.2 & & 43.9 & 64.7\\
\hline
& \multirow{2}{*}{BERT (UMLS pre-trained)} & 92.0 & 95.3 & & 93.0 & 95.3 & & 96.3 & 97.7 & & & & & 59.5 & 76.8 \\
\\
& \multirow{2}{*}{BioBERT v1.1 (UMLS pre-trained)} & 91.7 & 94.4 & & 93.1 & \textbf{95.7} & & \textbf{96.8} & 97.8 & & 72.4 & & & 63.7 & 75.3 \\
\\
& \multirow{2}{*}{BioClinicalBERT (UMLS pre-trained)} & 90.7 & 95.2 & & 93.0 & 95.9 & & 96.6 & 97.8 & &  & & & 62.1 & 75.7 & & \\
\\
& \multirow{2}{*}{BlueBERT (UMLS pre-trained)} & 90.8 & 94.0 & & 93.5 & 96.0 \\
\\
& \multirow{2}{*}{SciBERT (UMLS pre-trained)} & 92.5 & 95.1 & & 93.5 & 95.4  & & 96.5 & \textbf{98.0} & &  & & & 65.0 & 77.5  \\
\\
& \multirow{2}{*}{PubMedBERT (UMLS pre-trained)} & \textbf{93.5} & \textbf{95.7} & & \textbf{93.5} & \textbf{95.7} & & 96.5 & 97.8 & & & & & \textbf{65.8} & \textbf{78.4} \\
\\
\bottomrule
\end{tabular}
    \caption{Compare various base models before and after self-alignment pre-training on UMLS.}
    \label{tab:compare_base}
\end{table*}

\subsection{Qualitatively examine how pre-training has changed the semantic space of BERT}

\textbf{TODO:}\\
1. print some nearest neighbour's list of some selected synonyms \\
2. visualise embeddigns of some concepts using T-SNE. compare before and after pre-training


==> backups/intro.tex <==

\section{Introduction}
\label{sec:intro}
%Medical concept mentions can be spotted in various contexts, including but not limited to scientific papers, clinical notes and online forums. Automatic recognition of concept mentions is thus of great importance for facilitating scientific studies \& discoveries, enhancing clinical care procedures \zm{as well as} monitoring people's health quality in online communities. %In this paper we study Medical Concept Normalisation (MCN), i.e. the task of linking textual mentions to standard medical \zm{concepts (vocabulary/ontology)}.
%The task of Medical Concept Normalisation (MCN) is to link textual mentions in the context to concepts in standard medical terminology (e.g. vocabulary/ontology in SNOMED CT), which is the main focus of this paper.
Medical concept normalisation has been widely used in handling search queries in medical information systems, monitoring health quality in social media, processing clinical documents\zmc{citation?} and etc. It is of great importance for knowledge discovery in the biomedical domain.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/eacl_front_graphs.pdf}
    \caption{The embedding space t-SNE visualisation of PubMedBert \& SapBert where SapBert is further pre-trained on UMLS synonyms using PubMedBert as the base model. It can be observed that without self-alignment pre-training, biomedical names of different concepts are hard to separate from each other in the heterogeneous embedding space. After the pre-training, concepts' synonyms are self-aligned and form compact circles where names of different concepts live in distinct locations in the embedding space.}
    \label{fig:front}
\end{figure*}

The heterogeneous naming of biomedical concepts pose a major challenge to MCN. Names with completely different surface forms can have identical meanings, causing great challenges to semantic representations. For example, %the medication \emph{6-mercaptopurine} is also often referred to as \emph{6MP} (abbreviation) or \emph{Purinethol} (brand name).
the medication \emph{Hydroxychloroquine} (CUI: C0020336) is often referred to as \emph{Oxichlorochine} (alternative name), \emph{HCQ} (social media) and \emph{Plaquenil} (brand name). These cannot be easily represented with off-the-shelf *BERT as suggedted in Fig...(T-SNE visualisation of BioBert \& SapBert).
To mitigate the challenge posed by heterogeneous naming, prior works adopt complex text pre-processing pipelines. \citet{ji2020bert, sung2020biomedical} use spelling checking heuristics, abbreviation resolution toolkits and etc. Though being sophisticated, these rule-based systems can hardly cover all the variations of biomedical names. To solve the aforementioned obstacles, we propose to pre-train a Transformer-based language model on a very-large-scale biomedical knowledge graph, i.e. UMLS, 
to help learn the semantic representation for biomedical names. UMLS as the interlingua of biomedical ontologies contain comprehensive collections of biomedical synonyms in various forms and is thus an ideal external knowledge source for enhancing neural language model's semantic representations in the biomedical domain. The current UMLS 2020AA\zmc{citation or footnote?} has more than 4 million concepts and 10 million synonyms which stem from over 150 controlled vocabularies including MeSH, SNOMED CT, RxNorm, Gene Ontology and OMIM.\footnote{{\scriptsize \url{https://www.nlm.nih.gov/research/umls/knowledge_sources/metathesaurus/release/statistics.html}}} It is the largest single ontology of biomedical concepts.

Working with a knowledge graph with millions of concepts is non-trivial. %Directly applying such heavy machinery on UMLS is both memory \& training time infeasible. 
This has been a long-standing challenge for MCN systems. Recent neural MCN systems often adopt a two-stage pipeline where in the first stage the system generates possible candidates and in the second stage a neural model reranks the candidates. \citet{xu-etal-2020-generate, ji2020bert} leverage traditional string matching systems (such as Lucene and BM25)  to generate candidates while \citep{sung2020biomedical} use a hybrid of TF-IDF and BERT features to search for candidates. However, such generate-and-rerank framework \zmc{generate-and-rerank or two-stage pipeline? It is better to unify these two concepts.} is still difficult to scale especially for pre-training purposes. We propose to pre-train BERTs on UMLS with a self-alignment objective \zm{that groups \zmc{Is `predict' or `rank' more precise than`group'?}} synonyms of the same concept using a metric learning loss. We show that with a well-crafted non-parametric metric learning formulation, an end-to-end Transformer-based language model is sufficient to perform well on the MCN task. Our \textbf{S}elf-\textbf{a}ligning \textbf{p}retrained \textbf{BERT} (SapBERT), completely skips the candidate generation phase and does not contain a string-matching module, nonetheless showing comparable or better performance on multiple benchmarks without any finetuning on specific MCN datasets. When compared with other domain-pretrained contextual models (e.g. BioBERT and SciBERT), SapBERT can outperform them by as much as more than 20\% on top-1 accuracy across different benchmarks.

==> backups/method.tex <==
\section{Method: Self-Alignment Pre-training}\label{sec:method}
\fl{I shifted most of Zaiqiao's abstract here to motivate our methodology part.}
Masked language models pre-trained with biomedical corpora (such as SciBERT and BioBERT) have shown better performance in biomedical mining tasks than models pre-trained with only general domain corpora (e.g. the vanilla BERT). However, learning from distributional semantics in corpora does not equip the pre-trained models with fine-grained expert knowledge which is essential in performing downstream tasks such as MCN. 
% In particular, it requires a model to identify the rich synonyms among the biomedical concepts.
% the masked-word pre-training scheme adopted by these models that predicts randomly masked words in a sequence still neglect the rich synonyms among the biomedical concepts.
We design our pretraining scheme to leverage ULMS by learning to align a biomedical name with its synonyms defined in the knowledge base. We call this process self-alignment. In the following we introduce a consistent metric learning framework that is suitable for both conducting self-alignment pre-training a contextual model on UMLS synonyms and also finetuning one tailored for specific data sets.

\subsection{Problem definition} 
Let $(x, y)\in \mathcal{X} \times \mathcal{Y}$ denote a tuple of a name and its label (e.g. CUIs for UMLS names) where $\mathcal{X}, \mathcal{Y}$ are the collections of all names and their labels in the training set (for pre-training, $\mathcal{X} \times \mathcal{Y}$ is the all synonyms in UMLS; for finetuning, it is the concatenation of training data \& reference ontology). Given any pair of tuples $(x_i, y_i),(x_j, y_j) \in \mathcal{X}\times \mathcal{Y}$, the goal of self-alignment to learn a function $f(\cdot;\theta): \mathcal{X} \rightarrow \mathbb{R}^d$ parameterised by $\theta$ where cosine $\langle f(x_i),f(x_j) \rangle$ can be used to estimate the similarity of $x_i$ and $x_j$. $\langle f(x_i), f(x_j)\rangle$ should be high if $x_i,x_j$ are synonyms (i.e. $y_i=y_j$) and low if they are not (i.e. $y_i\neq y_j$). In this study, $f$ is instantiated with a BERT and the output at \texttt{[CLS]} token from BERT is regarded as the representation of the input. 

\subsection{Learning scheme}
During learning process, mini-batch training is adopted. Let $\mathcal{X}_b \times \mathcal{Y}_b \subseteq \mathcal{X} \times \mathcal{Y}$ be the batched names and their labels. We will first conduct an online mining procedure to select informative pairs of training samples and then send them to a pairwise metric learning loss function for learning. We explain them respectively in the following.

\stitle{Online hard pairs generation.} Online sample mining finds hard positive/negative pairs or triplets within the mini-batch for efficient training. We use a hard triplet mining condition to filter out ``easy positive \& negatives'' and identify the most informative  training triplets. Specifically, we construct all possible triplets for all names within the mini-batch where each triplet is in the form of $(x_a, x_p, x_n)$. Here $x_a$ is called ``anchor'', an arbitrary name in the mini-batch; $x_p$ is called a ``positive'' of the anchor (i.e. $y_a=y_p$) and $x_n$ is called a ``negative'' of $x_a$ (i.e. $y_a \neq y_n$). Among the constructed triplets, we select out all triplets that violate the following condition:
\begin{equation}
    \|f(x_a)-f(x_p)\|_2 <  \|f(x_a)-f(x_n)\|_2 + \lambda.
\end{equation}
where $\lambda$ is a pre-set margin. In other words, we only consider triplets with the negative closer to the positive by a margin of $\lambda$. We call them ``hard triplets'' as their original representations were very far from correct. Every hard triplet contributes one hard positive pair $(x_a,x_p)$ and one hard negative pair $(x_a,x_n)$. We collect all such positive \& negative pairs and denote them as $\mathcal{P},\mathcal{N}$. A similar but not identical triplet mining condition was used by \citet{schroff2015facenet} for face recognition in which they only used it for selecting hard negative samples.

\stitle{Loss function.} We then compute the pairwise cosine similarity of all the names' BERT representations and obtain a similarity matrix $\mathbf{S}\in\mathbb{R}^{|\mathcal{X}_b|\times |\mathcal{X}_b|}$ where each entry $\mathbf{S}_{ij}$ corresponds to the representation cosine similarity between the $i$-th name in the $j$-th name in the mini-batch.  A state-of-the-art metric learning loss called Multi-Similarity loss (MS loss) by \citet{wang2019multi} is adopted for learning from the positive and negative pairs:
\begin{equation}
    \begin{split}
\mathcal{L} = \frac{1}{|\mathcal{X}_b|}\sum_{i=1}^{|\mathcal{X}_b|} \Bigg(\frac{1}{\alpha}\log\Big(1+\sum_{n\in \mathcal{N}_i } e^{\alpha (\mathbf{S}_{in} -\epsilon )}\Big) \\
 + \frac{1}{\beta} \log \Big(1+\sum_{p \in \mathcal{P}_{i}} e ^{ - \beta (\mathbf{S}_{ip} -\epsilon)} \Big)\Bigg) ,
\label{eq:loss}
\end{split}
\end{equation}
where $\alpha,\beta$ are temperature scales; $\epsilon$ is an offset applied on the similarity matrix; $\mathcal{P}_i,\mathcal{N}_i$ are indices of positive and negative samples of the anchor $i$. 

\stitle{Why is MS loss better?} Previous MCN models that leverage UMLS synonyms adopted other forms of pairwise losses. \citet{phan2019robust} used a simple cosine loss and \citet{schumacher2020clinical} used a triplet loss. We will show in experiments that applying such naive loss functions on the full UMLS does not yield optimal pre-training results (actually, there is a very significant gap between theirs' and ours). The main reason is that MS loss leverages similarities among and between positives \& negative to reweight the importance of sample pairs. The most informative pairs will be assigned with more gradients in training and thus can make full use of information stored in data. A cosine loss does not consider similarities among samples in any form while triplet loss assigns equal weights to every sample in the mini-batch, both leading to insufficient learning. A detailed gradient analysis for comparing such three losses can be found in appendix.

==> backups/related_work.tex <==

\section{Related Work}
\label{sec:related_work}

Our work is connected to two major topics in NLP, \zm{namely medical concept normalisation and pre-training medical language representations}. %Each has a large body of work which we can only provide as a highly selected summary.


\subsection{Medical Concept Normalisation}
%\footnote{Entity linking (EL) from free-text usually requires Named Entity Recognition (NER) and Named Entity Normalisation (NEN) which are two foundational text processing tasks. MCN is essentially the NEN step in the Medical Entity Linking pipeline.Recently, end-to-end neural EL systems \citep{kolitsas2018end,peters2019knowledge} have also emerged but we focus on NEN step in this study.}

Solutions to MCN can be generally divided into hand-crafted rule-based systems, classification-based neural models and generate-and-rank systems \zmc{It is better to unify ``models" and ``systems" to the some expression (e.g. ``methods")}. 
% Rule-based systems combine string matching heuristics and dictionary look-up in a careful manner. Popular rule-based systems include MetaMaps \citep{aronson2001effective}, cTakes \citep{savova2010mayo} and Sieve-based matching system \citep{dsouza-ng-2015-sieve}. 
While being robust baselines, popular rule-based systems include MetaMaps \citep{aronson2001effective}, cTakes \citep{savova2010mayo} and Sieve-based matching system \citep{dsouza-ng-2015-sieve} struggle to cover all variations of biomedical names (e.g. biomedical name mentions in the social media \citep{cometa}).
Classification-based neural systems demonstrate strong performance against rule-based ones, especially in the social media domain, by learning semantic representations of biomedical names. \citet{limsopatham2016normalising} applied the CNN-based methods while \citet{tutubalina2018medical,miftahutdinov2019deep} combined the TF-IDF features with GRU or BERT representations.

% However, pure neural systems with a multi-class classification-based objective cannot handle a large reference ontology. 

To cope with a large reference ontology, most of the recent studies adopted generate-and-rank systems that first generate a small list of possible candidates to reduce the output space and then leverage the neural models to rerank these candidates. 
%A plethora number of methods have been adopted for candidate generation. 
\citet{li2017cnn} use sieve-based rules, similar to \citet{d2015sieve}, to generate candidates and then use a CNN-based model to conduct a reranking. \citet{leaman2013dnorm,murty2018hierarchical} leverage the TF-IDF similarity scores and then apply the neural models on the candidates only. BioSyn proposed by \citep{sung2020biomedical} adopts a similar pipeline but leverages the combination of BERT features and TF-IDF features to propose candidates and train the system by marginalising positive samples. \citet{ji2020bert} 
leverage BM25 to produce candidates and use BERT to rerank them. \citet{xu-etal-2020-generate} adopt a similar architecture as \citet{ji2020bert} with the difference that they use the Lucene-based string matching system instead and they also predict semantic type of a concept during training, acting as a regularisation to the original learning objective. 

Our proposed SapBert breaks the curse of scale by producing high quality low-dimensional neural representations. SapBert finds the target canonical concept with a simple nearest neighbour search (NNS). It performs on par or better than the SOTA MCN systems even without training on scientific language MCN data sets. For social media MCN data sets, SapBert outperforms the SOTAs after a finetuning on the training sets.

\subsection{Pre-training medical language representations on structured data}
%In the medical domain,
%Injecting structured knowledge from knowledge graphs have always been a relevant topic for language representation learning as distributional-semantics-based objectives does not fully capture the abundant knowledge stored in semantic lexicons  \citep{faruqui2015retrofitting}. This is especially true in the biomedical domain where very ... experts. 
Conceptually similar to our idea, \citet{alawad2018retrofitting} retrofit word embeddings on a subset of UMLS and observed improvement when applied on information extraction tasks. More recetly, \citet{phan2019robust} train char/word embeddings + BiLSTM to group synonyms in UMLS. Like ours, their model produces generic medical names and can operate without finetuning on specific data sets. However, they did not use a contextual model (e.g. BERT) and optimises a naive cosine similarity objective function. We will empirically show that SapBert performs significantly better than theirs and apply the same cosine objective for BERT, on a very large scale, does not produce high quality semantic representations.
\citet{schumacher2020clinical} also points out that UMLS synonyms can serve as additional training data for their MCN model. However, their pre-training operates on mentions with contexts and thus could only leverage a subset of UMLS where contexts exist. \citet{zhang2020learning} train an LSTM-based language model on UMLS with a knowledge graph embedding objective. It encodes an entity along with its context and is thus not directly comparable to SapBert. Note that there are also works on directly embedding UMLS KG as entity representations but they cannot be applied to MCN and are thus out of the scope of our discussion.

%(In the general domain...
%\citep{faruqui2015retrofitting})

\section{Method: Self-Alignment Pre-training}
\fl{I shifted most of Zaiqiao's abstract here to motivate our methodology part.}
Masked language models pre-trained with biomedical corpora (such as SciBERT and BioBERT) have shown better performance in biomedical mining tasks than models pre-trained with only general domain corpora (e.g. the vanilla BERT). However, learning from distributional semantics in corpora does not equip the pre-trained models with fine-grained expert knowledge which is essential in performing downstream tasks such as MCN. 
% In particular, it requires a model to identify the rich synonyms among the biomedical concepts.
% the masked-word pre-training scheme adopted by these models that predicts randomly masked words in a sequence still neglect the rich synonyms among the biomedical concepts.
We design our pretraining scheme to leverage ULMS by learning to align a biomedical name with its synonyms defined in the knowledge base. We call this process self-alignment. In the following we introduce a consistent metric learning framework that is suitable for both conducting self-alignment pre-training a contextual model on UMLS synonyms and also finetuning one tailored for specific data sets.

\subsection{Problem definition} 
Let $(x, y)\in \mathcal{X} \times \mathcal{Y}$ denote a tuple of a name and its label (e.g. CUIs for UMLS names) where $\mathcal{X}, \mathcal{Y}$ are the collections of all names and their labels in the training set (for pre-training, $\mathcal{X} \times \mathcal{Y}$ is the all synonyms in UMLS; for finetuning, it is the concatenation of training data \& reference ontology). Given any pair of tuples $(x_i, y_i),(x_j, y_j) \in \mathcal{X}\times \mathcal{Y}$, the goal of self-alignment to learn a function $f(\cdot;\theta): \mathcal{X} \rightarrow \mathbb{R}^d$ parameterised by $\theta$ where cosine $\langle f(x_i),f(x_j) \rangle$ can be used to estimate the similarity of $x_i$ and $x_j$. $\langle f(x_i), f(x_j)\rangle$ should be high if $x_i,x_j$ are synonyms (i.e. $y_i=y_j$) and low if they are not (i.e. $y_i\neq y_j$). In this study, $f$ is instantiated with a BERT and the output at \texttt{[CLS]} token from BERT is regarded as the representation of the input. 

\subsection{Learning scheme}
During learning process, mini-batch training is adopted. Let $\mathcal{X}_b \times \mathcal{Y}_b \subseteq \mathcal{X} \times \mathcal{Y}$ be the batched names and their labels. We will first conduct an online mining procedure to select informative pairs of training samples and then send them to a pairwise metric learning loss function for learning. We explain them respectively in the following.

\stitle{Online hard pairs generation.} Online sample mining finds hard positive/negative pairs or triplets within the mini-batch for efficient training. We use a hard triplet mining condition to filter out ``easy positive \& negatives'' and identify the most informative  training triplets. Specifically, we construct all possible triplets for all names within the mini-batch where each triplet is in the form of $(x_a, x_p, x_n)$. Here $x_a$ is called ``anchor'', an arbitrary name in the mini-batch; $x_p$ is called a ``positive'' of the anchor (i.e. $y_a=y_p$) and $x_n$ is called a ``negative'' of $x_a$ (i.e. $y_a \neq y_n$). Among the constructed triplets, we select out all triplets that violate the following condition:
\begin{equation}
    \|f(x_a)-f(x_p)\|_2 <  \|f(x_a)-f(x_n)\|_2 + \lambda.
\end{equation}
where $\lambda$ is a pre-set margin. In other words, we only consider triplets with the negative closer to the positive by a margin of $\lambda$. We call them ``hard triplets'' as their original representations were very far from correct. Every hard triplet contributes one hard positive pair $(x_a,x_p)$ and one hard negative pair $(x_a,x_n)$. We collect all such positive \& negative pairs and denote them as $\mathcal{P},\mathcal{N}$. A similar but not identical triplet mining condition was used by \citet{schroff2015facenet} for face recognition in which they only used it for selecting hard negative samples.

\stitle{Loss function.} We then compute the pairwise cosine similarity of all the names' BERT representations and obtain a similarity matrix $\mathbf{S}\in\mathbb{R}^{|\mathcal{X}_b|\times |\mathcal{X}_b|}$ where each entry $\mathbf{S}_{ij}$ corresponds to the representation cosine similarity between the $i$-th name in the $j$-th name in the mini-batch.  A state-of-the-art metric learning loss called Multi-Similarity loss (MS loss) by \citet{wang2019multi} is adopted for learning from the positive and negative pairs:
\begin{equation}
    \begin{split}
\mathcal{L} = \frac{1}{|\mathcal{X}_b|}\sum_{i=1}^{|\mathcal{X}_b|} \Bigg(\frac{1}{\alpha}\log\Big(1+\sum_{n\in \mathcal{N}_i } e^{\alpha (\mathbf{S}_{in} -\epsilon )}\Big) \\
 + \frac{1}{\beta} \log \Big(1+\sum_{p \in \mathcal{P}_{i}} e ^{ - \beta (\mathbf{S}_{ip} -\epsilon)} \Big)\Bigg) ,
\label{eq:loss}
\end{split}
\end{equation}
where $\alpha,\beta$ are temperature scales; $\epsilon$ is an offset applied on the similarity matrix; $\mathcal{P}_i,\mathcal{N}_i$ are indices of positive and negative samples of the anchor $i$. 

\stitle{Why is MS loss better?} Previous MCN models that leverage UMLS synonyms adopted other forms of pairwise losses. \citet{phan2019robust} used a simple cosine loss and \citet{schumacher2020clinical} used a triplet loss. We will show in experiments that applying such naive loss functions on the full UMLS does not yield optimal pre-training results (actually, there is a very significant gap between theirs' and ours). The main reason is that MS loss leverages similarities among and between positives \& negative to reweight the importance of sample pairs. The most informative pairs will be assigned with more gradients in training and thus can make full use of information stored in data. A cosine loss does not consider similarities among samples in any form while triplet loss assigns equal weights to every sample in the mini-batch, both leading to insufficient learning. A detailed gradient analysis for comparing such three losses can be found in appendix.

==> includes/related_works.tex <==
% To cite
% EMNLP 2020
% BioMegatron
% A Knowledge-driven Generative Model for Multi-implication Chinese Medical Procedure Entity Normalization
% https://www.aclweb.org/anthology/2020.emnlp-main.116.pdf
